High-performance stock index trading: making effective use of a deep LSTM neural network

We present a deep long short-term memory (LSTM)-based neural network for predicting asset prices, together with a successful trading strategy for generating profits based on the model's predictions. Our work is motivated by the fact that the effectiveness of any prediction model is inherently coupled to the trading strategy it is used with, and vise versa. This highlights the difficulty in developing models and strategies which are jointly optimal, but also points to avenues of investigation which are broader than prevailing approaches. Our LSTM model is structurally simple and generates predictions based on price observations over a modest number of past trading days. The model's architecture is tuned to promote profitability, as opposed to accuracy, under a strategy that does not trade simply based on whether the price is predicted to rise or fall, but rather takes advantage of the distribution of predicted returns, and the fact that a prediction's position within that distribution carries useful information about the expected profitability of a trade. The proposed model and trading strategy were tested on the S&P 500, Dow Jones Industrial Average (DJIA), NASDAQ and Russel 2000 stock indices, and achieved cumulative returns of 340%, 185%, 371% and 360%, respectively, over 2010-2018, far outperforming the benchmark buy-and-hold strategy as well as other recent efforts.

==> bib.tex <==
\bibitem{Fama_French}
Eugene F. Fama, Kenneth R. French,
Common risk factors in the returns on stocks and bonds,
Journal of Financial Economics, Volume 33, Issue 1, 1993, Pages 3-56,
ISSN 0304-405X, https://doi.org/10.1016/0304-405X(93)90023-5

\bibitem{yahoofinance}
Yahoo Finance, 2018, Available at: https://finance.yahoo.com/quote/
[Accessed 1st May 2018]

\bibitem{image_recongnition_ILSVRC}
Olga Russakovsky*, Jia Deng*, Hao Su, Jonathan Krause, Sanjeev Satheesh, Sean Ma, Zhiheng Huang, Andrej Karpathy, Aditya Khosla, Michael Bernstein, Alexander C. Berg and Li Fei-Fei. (* = equal contribution) \emph{ImageNet Large Scale Visual Recognition Challenge}. IJCV, 2015

\bibitem{image_recongition_convolutional_networks}
Gao Huang, Zhuang Liu, Kilian Q. Weinberger,
Densely Connected Convolutional Networks,
CoRR,Volume 1608.06993, 2016, 

\bibitem{Dropout}
 Y. Gal, Z Ghahramani,
A Theoretically Grounded Application of Dropout in Recurrent Neural Networks, 2016, https://arxiv.org/abs/1512.05287
 
\bibitem{AlphaGo}
David Silver, Julian Schrittwieser, Karen Simonyan, Ioannis Antonoglou, Aja Huang, Arthur Guez, Thomas Hubert, Lucas Baker, Matthew Lai, Adrian Bolton, Yutian Chen, Timothy Lillicrap, Fan Hui, Laurent Sifre, George van den Driessche, Thore Graepel, Demis Hassabis,
Mastering the game of Go without human knowledge, Nature, 2017/10/18/ online, 550, 354, Macmillan Publishers Limited, part of Springer Nature, http://dx.doi.org/10.1038/nature24270. 
 
\bibitem{Bao}
Bao W, Yue J, Rao Y (2017) A deep learning framework for financial time series using stacked autoencoders and long-short term memory. PLoS ONE 12(7): e0180944. https://doi.org/10.1371/journal.pone.0180944

\bibitem{LSTM_origin}
Hochreiter, S., Schmidhuber, Jü. (1997). Long short-term memory. Neural computation, 9, 1735--1780. 


\bibitem{NMT}
Wu, Y., Schuster, M., Chen, Z., Le, Q. V., Norouzi, M., Macherey, W., Krikun, M., Cao, Y., Gao, Q., Macherey, K., others (2016). Google's neural machine translation system: Bridging the gap between human and machine translation. arXiv preprint arXiv:1609.08144. 

\bibitem{nmt_recent_advances}
Mia Xu Chen, Orhan Firat, Ankur Bapna, Melvin Johnson, Wolfgang Macherey, George Foster, Llion Jones, Niki Parmar, Mike Schuster, Zhifeng Chen, Yonghui Wu, Macduff Hughes, The Best of Both Worlds: Combining Recent Advances in Neural Machine Translation, Journal CoRR, Volume 1804.09849, 2018.


\bibitem{krauss_do_huck}
Krauss, Christopher $\&$ Do, Xuan Anh $\&$ Huck, Nicolas, 2016, Deep neural networks, gradient-boosted trees, random forests: Statistical arbitrage on the S$\&$P 500, FAU Discussion Papers in Economics 03/2016, Friedrich-Alexander University Erlangen-Nuremberg, Institute for Economics.

\bibitem{feng_He_Polson}
Feng, G., He, J. $\&$ Polson, N. G. (2018). Deep Learning for Predicting Asset Returns. CoRR, abs/1804.09314. 

\bibitem{gu_Kelly_Xiu}
Gu, Shihao and Kelly, Bryan T. and Xiu, Dacheng,
Empirical Asset Pricing via Machine Learning, June 11, 2018, Chicago Booth Research Paper No. 18-04. Available at SSRN: https://ssrn.com/abstract=3159577 or http://dx.doi.org/10.2139/ssrn.3159577


\bibitem{Nelson_Pereira_Oliveira}
D. M. Q. Nelson, A. C. M. Pereira and R. A. de Oliveira,
Stock market's price movement prediction with LSTM neural networks,
2017, International Joint Conference on Neural Networks (IJCNN), Anchorage, AK, 2017, pp. 1419-1426.
doi: 10.1109/IJCNN.2017.7966019

\bibitem{Zhong_Enke}
Zhong, X. $\&$ Enke, D. (2017). Forecasting daily stock market return using dimensionality reduction.. Expert Syst. Appl., 67, 126-139. 

\bibitem{Sethi_Treleaven_Rollin}
Sethi, M., Treleaven, P. C. $\&$ Rollin, S. D. B. (2014). Beating the S$\&$P 500 index - A successful neural network approach.. IJCNN (p./pp. 3074-3077), : IEEE. ISBN: 978-1-4799-6627-1 
   
\bibitem{fidelity}
Fidelity, 2018, \emph{About short selling}, [Online] Available at:  https://www.fidelity.com/learning-center/trading-investing/trading/about-short-selling [Accessed 6 July 2018]

\bibitem{KraussFisher}
Fischer, T. $\&$ Krauss, C. (2018). Deep learning with long short-term memory networks for financial market predictions. European Journal of Operational Research, 270, 654-669. 

\bibitem{ModAugNet}
Y. Baek, Ha Young Kim, ModAugNet: A new forecasting framework for stock market index value with an overfitting prevention LSTM module and a prediction LSTM module, Expert Systems with Applications, (2018), Volume 113, Pages 457-480, doi: https://doi.org/10.1016/j.eswa.2018.07.019

\bibitem{EMD2FNN}
F. Zhou, H. Zhou, Z. Yang, L. Yang, EMD2FNN: A strategy combining empirical mode decomposition and factorization machine based neural network for stock market trend prediction, Expert Systems with Applications, (2019), Volume 115, Pages 136-151, doi: https://doi.org/10.1016/j.eswa.2018.07.065

\bibitem{OmerMurat_Algorithmic}
Sezer, Omer, Ozbayoglu, Murat, Algorithmic Financial Trading with Deep Convolutional Neural Networks: Time Series to Image Conversion Approach, Applied Soft Computing,  (2018), 70. 10.1016/j.asoc.2018.04.024

\bibitem{investopedia}
Investopedia, 2018, Dictionary of Words, [Online] Available at: https://www.investopedia.com/ [Accessed 28 July 2018]

% @misc{fidelity,
%   Author = "Fidelity",
%   Title  = "About short selling",
%   Note   = "\url{https://www.fidelity.com/learning-center/trading-investing/trading/about-short-selling}[Accessed: 6 July 2018]",
%   year = 2018,
% }

% @conference{Nelson_Pereira_Oliveira,
% 	author = "D. M. Q. Nelson and A. C. M. Pereira and R. A. de Oliveira",
%     title = "Stock market's price movement prediction with LSTM neural networks",
%     journal  = "International Joint Conference on Neural Networks (IJCNN), Anchorage, AK",
%     year = "2017",
%     pages = "1419-1426",
%     doi  = "10.1109/IJCNN.2017.7966019"
    
% }

% @inproceedings{Dropout,
%   author    = {Yarin Gal andZoubin Ghahramani},
%   title     = {A Theoretically Grounded Application of Dropout in Recurrent Neural Networks},
%   booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference on Neural Information Processing Systems, Barcelona, Spain},
%   pages     = {1019--1027},
%   year      = {2016},
%   month     = "December",
%   url       = {http://papers.nips.cc/paper/6241-a-theoretically-grounded-application-of-dropout-in-recurrent-neural-networks},
% }


